LAC: Latent Action Composition for Skeleton-based Action Segmentation

Skeleton-based action segmentation requires recognizing composable actions in untrimmed videos. Current approaches decouple this problem by first extracting local visual features from skeleton sequences and then processing them by a temporal model to classify frame-wise actions. However, their performances remain limited as the visual features cannot sufficiently express composable actions. In this context, we propose Latent Action Composition (LAC), a novel self-supervised framework aiming at learning from synthesized composable motions for skeleton-based action segmentation. LAC is composed of a novel generation module towards synthesizing new sequences. Specifically, we design a linear latent space in the generator to represent primitive motion. New composed motions can be synthesized by simply performing arithmetic operations on latent representations of multiple input skeleton sequences. LAC leverages such synthesized sequences, which have large diversity and complexity, for learning visual representations of skeletons in both sequence and frame spaces via contrastive learning. The resulting visual encoder has a high expressive power and can be effectively transferred onto action segmentation tasks by end-to-end fine-tuning without the need for additional temporal models. We conduct a study focusing on transfer-learning and we show that representations learned from pre-trained LAC outperform the state-of-the-art by a large margin on TSU, Charades, PKU-MMD datasets.

==> section/introduction.tex <==
\section{Introduction}
\input{iccv2023AuthorKit/figures/intro}
%Human-centric activity recognition is a crucial task in real-world video understanding~\cite{3dcnn, Carreira_2017_CVPR, 3d-resnet, slow-fast, x3d, Ryoo2020AssembleNetAM, li2021ctnet, Wang_2021_CVPR, arnab2021vivit}. In this context, skeleton data (\ie, 2D/3D human keypoints) plays an important role as it have proved to be more robust to content changes (\eg, camera viewpoints, subject appearance, etc.) compared to other modalities. %such as RGB videos and optical flows.
%%methods adopting spatio-temporal Convolutional Neural Networks (CNNs)~\cite{3dcnn, Carreira_2017_CVPR, 3d-resnet, slow-fast, x3d, Ryoo2020AssembleNetAM, li2021ctnet, Wang_2021_CVPR} or Transformer-based~\cite{arnab2021vivit} networks to extract features from RGB videos and optical flows~\cite{two-stream, c-2stream}, skeleton-based methods~\cite{Caetano2019SkeletonIR, Yan2018SpatialTG, 2sagcn2019cvpr, res-gcn, unik, topology_2021_ICCV, duan2021revisiting, yang2022via} relying on 2D/3D human keypoints,
%Due to the strong representational power of skeleton data, the study of approaches able to recognize activities directly from 2D/3D skeletons has gained increasing attention~\cite{Caetano2019SkeletonIR, Yan2018SpatialTG, 2sagcn2019cvpr, res-gcn, unik, topology_2021_ICCV, duan2021revisiting, yang2022via}. Moreover, human skeletons usually convey significant information that is complementary to other modalities such as RGB and optical flow~\cite{Das_2019_ICCV, das2020vpn, das2021vpn+, duan2021revisiting}.
%
%


Human-centric activity recognition is a crucial task in real-world video understanding. In this context, \textit{skeleton data} that can be represented by 2D or 3D human keypoints plays an important role, as it is complementary to other modalities such as RGB~\cite{3dcnn, Carreira_2017_CVPR, 3d-resnet, slow-fast, x3d, Ryoo2020AssembleNetAM, li2021ctnet, Wang_2021_CVPR, arnab2021vivit} videos and optical flow~\cite{two-stream, c-2stream}. As representation of human motions has witnessed robustness \wrt content changes related to camera viewpoints and subject appearances, the study of recognizing activities directly from 2D/3D skeletons has gained increasing attention~\cite{Du2015HierarchicalRN, DING-jvcir, Caetano2019SkeletonIR, Yan2018SpatialTG, 2sagcn2019cvpr, aaai2021multiscale, res-gcn, unik, topology_2021_ICCV, graphscattering, duan2021revisiting, yang2022via, Dai_2022_PAMI}. While current approaches~\cite{Du2015HierarchicalRN, DING-jvcir, Caetano2019SkeletonIR, Yan2018SpatialTG, 2sagcn2019cvpr, aaai2021multiscale, res-gcn, unik, topology_2021_ICCV, graphscattering, duan2021revisiting, yang2022via} have achieved remarkable success, such approaches often focus on \textit{trimmed videos} containing \textit{single actions}, which constitutes a highly simplified scenario. Deviating from this, in this work, we tackle the challenging setting of \textit{action segmentation in untrimmed videos based on skeleton sequences}.



%Skeleton-based approaches~\cite{Caetano2019SkeletonIR, Yan2018SpatialTG, 2sagcn2019cvpr, res-gcn, unik, topology_2021_ICCV, duan2021revisiting, yang2022via} typically focus on action classification for trimmed videos. In this paper, we focus on a more complex and challenging problem and we present a novel skeleton-based method for multi-label and frame-wise action classification (\ie, action segmentation) in untrimmed videos.
%
%%In this paper, deviating from current methods~\cite{Caetano2019SkeletonIR, Yan2018SpatialTG, 2sagcn2019cvpr, res-gcn, unik, topology_2021_ICCV, duan2021revisiting, yang2022via} which only focus on the action classification for trimmed videos, we present a novel skeleton-based method for multi-label and frame-wise action classification (\ie, action segmentation) in untrimmed videos.
%Such task is more challenging and complex, as multiple actions can be performed by the same subject and all the performed actions need to be identified and classified. In order to process the long-term features in untrimmed videos, current detection methods~\cite{lea2017temporal, TGM, superevent, Dai_2022_PAMI} apply temporal modeling on visual representations of the video which are pre-extracted along a sliding window by a pre-trained visual encoder. The performance thus highly relies on the representation capability of the pre-trained visual encoder. Unfortunately, current large-scale skeleton pre-training datasets~\cite{NTU-120, unik, Yan2018SpatialTG} contain only trimmed sequences and no composable (\ie, co-occurred) actions. Based on this observation, we hypothesize that the expressive power of skeleton action representations could be improved, especially for action segmentation downstream tasks, by constructing composable skeleton motions for training the visual encoder.
%%on trimmed datasets. 

In untrimmed videos, activities are composable \ie, motion performed by a person generally comprises multiple actions (co-occurrence), each with the duration of a few seconds. Towards modeling \textit{long-term dependency} among different actions, representative and expressive skeleton features are required. Current approaches~\cite{lea2017temporal, TGM, superevent, Dai_2022_PAMI} obtain such features through visual encoder such as AGCNs pre-trained on trimmed datasets. However, we found that due to lack of composable actions in such datasets, the performance of using such features in our setting is far from satisfactory. Towards addressing this issue, we propose to construct \textit{synthesized composable skeleton data} for training a more effective visual encoder, endowed with strong representability of subtle action details for action segmentation.



%In this paper, we propose Composable Motion Synthesis (LAC), a self-supervised skeleton action representation framework composed of a generative module and a contrastive module, as shown in Fig.~\ref{fig:intro}.


In this paper, we propose Latent Action Composition (LAC), a novel self-supervised framework aiming at synthesizing composable motion data for action segmentation. As shown in Fig.~\ref{fig:intro} (left), our framework consists of two parts, a generative module and a contrastive module. 


%
%\begin{inparaenum}[(i)]
%\item 

The \textit{generative module} is based on an autoencoder that synthesizes skeleton motions combined from multiple videos. As the high-level motions are difficult to combine directly by the joint coordinates (\eg, `drink' and `sitdown'), LAC seeks to learn an action dictionary. Such action dictionary incorporates an orthogonal basis in the latent encoding space, containing two sets of directions. The first set named `Character' includes directions representing high-level static information of the skeleton sequence, for instance, viewpoints, body size, etc. The other set named `Motion' includes directions representing basic temporal information of the skeleton sequence, for instance, the dynamics of the action performed by the subject. The new skeleton sequence is generated via a linear combination of the learned `Character' and `Motion' directions. In the training stage, we adopt motion retargeting to train the autoencoder and the dictionary for a pair of input skeleton sequences. 
%Specifically, we swap their learned `Motion' and `Character' sets of their latent codes to generate (\ie, decode) skeleton sequences where subjects perform each other's action, while maintaining viewpoint and body size invariance. 
In the inference stage, we take multiple skeleton sequences as inputs and generate composable motions 
%with their respective `Character' parts 
 by combining their latent `Motion' sets.% in the latent codes.   
%\item 

%The contrastive module is designed to train an skeleton visual encoder~\cite{unik} that is invariant to data augmentations on a large-scale dataset using the composed skeleton sequences. 
The \textit{contrastive module} trains a skeleton visual encoder such as UNIK~\cite{unik} in a self-supervised manner without need for action labels. It is designed for the resulting visual encoder to be able to maximize the similarity of different skeleton sequences, that are obtained via data augmentation from the same original sequence, across large-scale datasets.
%The contrastive module trains a skeleton visual encoder such as UNIK~\cite{unik}, for instance. The contrastive module is designed so that the resulting visual encoder is able to maximize, across large-scale datasets, the similarity of different skeleton sequences that are obtained via data augmentation from the same original sequence.
%As the learned visual transformation dictionary contain the directions representing static `viewpoint' and `body size' transformations, we can generate a composable skeleton sequence in diffenrent viewpoints by modification of the corresponding magnitudes as the positive samples. 
Unlike current methods~\cite{ding2022motion, selfrgb_2021_huang, transformer2022selfsupervised, selfrgb_2021_huang, Sun_2021_ICCV, ConNTU, Mao_2022_CMD, yang2022via} that perform contrastive learning for the video-level representations, we perform contrastive learning also on an additional frame space to finely maximize the per-frame similarities between the positive samples. Subsequently, the so-trained frame-level skeleton visual encoder is transferred and retrained on action segmentation datasets~\cite{Dai_2022_PAMI, Sigurdsson2016HollywoodIH}.
%\end{inparaenum}

To assess the performance of LAC, we train LAC on the large-scale dataset Posetics~\cite{unik} and we evaluate the quality of the learned skeleton representations by fine-tuning onto unseen daily action segmentation datasets (\eg, TSU~\cite{Dai_2022_PAMI}, Charades~\cite{Sigurdsson2016HollywoodIH}, PKU-MMD~\cite{liu2017pku}). Experimental analyses confirm that motion composition and contrastive learning can significantly increase the expressive power of the visual encoder. The fine-tuning results outperform state-of-the-art accuracy obtained by temporal modeling.
%on pre-extrated visual representations. 

In summary, the contributions of this paper are the following:
\begin{inparaenum}[(i)]
\item We introduce LAC, a novel generative and contrastive framework to synthesize complex motions and improve the skeleton action representation capability.
\item In the generative module, we introduce a novel 
%and interpretive 
Linear Action Decomposition (LAD) mechanism to represent high-level motion features by an orthogonal basis. The motion features for multiple skeleton sequences can thus be linearly combined in the latent space. 
\item In the contrastive module, we propose to perform contrastive learning of the representations in both video space and frame space to better generalize to frame-wise action segmentation tasks.
%\item We set new state-of-the-art performance based on skeleton sequences for self-supervised transfer-learning on real-world action segmentation datasets. 
\item We conduct a study and show that pre-training LAC on Posetics and transferring it onto an unseen target untrimmed video dataset represents a generic and effective methodology for action segmentation.

\end{inparaenum}

%As high-level motions are difficult to be combined directly,
%generative module
%To further adapt to densely labeled tasks, Contrastive module

%Untrimmed important, current work only single modality, skeleton advantage, people ignore, bu challenge : no composable in pretrain trimmed?
